The Medium is the Message: How Secure Messaging Apps Leak Sensitive Data to Push Notification Services

Like most modern software, secure messaging apps rely on third-party components to implement important app functionality. Although this practice reduces engineering costs, it also introduces the risk of inadvertent privacy breaches due to misconfiguration errors or incomplete documentation. Our research investigated secure messaging apps' usage of Google's Firebase Cloud Messaging (FCM) service to send push notifications to Android devices. We analyzed 21 popular secure messaging apps from the Google Play Store to determine what personal information these apps leak in the payload of push notifications sent via FCM. Of these apps, 11 leaked metadata, including user identifiers (10 apps), sender or recipient names (7 apps), and phone numbers (2 apps), while 4 apps leaked the actual message content. Furthermore, none of the data we observed being leaked to FCM was specifically disclosed in those apps' privacy disclosures. We also found several apps employing strategies to mitigate this privacy leakage to FCM, with varying levels of success. Of the strategies we identified, none appeared to be common, shared, or well-supported. We argue that this is fundamentally an economics problem: incentives need to be correctly aligned to motivate platforms and SDK providers to make their systems secure and private by default.

==> assets/tables/table_broken_promises-trinity.tex <==

\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{table*}[]\large
\centering
\resizebox{\textwidth}{!}

\begin{tabular}{S|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}} 
    \multicolumn{7}{S}{Table of Broken Promises} \\
    \toprule
    App Name & Message Content & Device IDs & User IDs & Name & Phone Number & Contacts \\
    \midrule
    Viber & & \frownie & \frownie & & & \frownie \\
    Wire & & \frownie & \frownie & & & \\
    Skype & \frownie & \frownie & \frownie & \frownie & & \\
    Snapchat & &  & \frownie & \frownie & & \frownie \\
    WeChat & \frownie & & \frownie & \frownie & & \frownie \\
    Discord & \frownie & & \frownie & \frownie & & \frownie \\
    JusTalk & \frownie & & \frownie & \frownie & & \frownie \\
    SafeUM & & & \frownie & & & \\
    YallaChat & & & \frownie & \frownie & & \frownie \\
    Comera & & & & & \frownie & \\
    \bottomrule
\end{tabular}

\caption{\textcolor{red}{Revised table/caption by Trinity} Promises made, promises broken. We observed that the apps that leaked data to Google via FCM had stated in their respective disclosure documents that this data would not be shared with any third parties. All such discrepancies are listed in this table.}
\label{tab:broken_promises}
\end{table*}


==> assets/tables/table_broken_promises.bkp.tex <==
% ===== NOTE =====
% This table was generated using the online tool:
% https://www.tablesgenerator.com/latex_tables
% To make any changes to this table:
% 1) Download the file *.tgn
% 2) Load *.tgn into the TablesGenerator tool
% 3) Make changes via the GUI
% 4) Copy/paste the generated latex output back into
%    this file, while preserving this comment
% 5) Change \begin{table}[] to \begin{table*}[]
%    so that the table floats to the top of the page
% 6) In TablesGenerator, save the table to a .tgn file
% 7) Upload the new *.tgn file to Overleaf so that 
%    everything is organized and versioned together
% ===== NOTE =====

\begin{table*}[t!]
\centering
\begin{tabular}{llcccccc}
\hline
\multirow{2}{*}{\textbf{App}}                                                &                                   & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Privacy\\ Strategy\end{tabular}}} & \multicolumn{5}{c}{\textbf{Observed Leakage to FCM}}                                                                                                     \\ \cline{4-8} 
                                                                             &                                   &                                                                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Message\\ Content\end{tabular}} & \textbf{Device IDs} & \textbf{User IDs} & \textbf{Name} & \textbf{Phone \#} \\ \hline
\href{https://play.google.com/store/apps/details?id=com.skype.raider}{Skype} & \multicolumn{1}{c}{(default)}     & none                                                                                 & \newmoon                                                           & \newmoon            & \newmoon          & \newmoon      & \fullmoon         \\
                                                                             & \multicolumn{1}{c}{(secret chat)} & e2ee                                                                                 & \fullmoon                                                          & \newmoon            & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.snapchat.android}{Snapchat}}          & e2ee                                                                                 & \fullmoon                                                          & \fullmoon           & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.viber.voip}{Viber}}                   & Push-to-Sync                                                                         & \fullmoon                                                          & \newmoon            & \newmoon          & \fullmoon     & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=jp.naver.line.android}{LINE}}             & e2ee                                                                                 & \fullmoon                                                          & \fullmoon           & \fullmoon         & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.discord}{Discord}}                    & none                                                                                 & \newmoon                                                           & \fullmoon           & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.tencent.mm}{WeChat}}                  & none                                                                                 & \newmoon                                                           & \fullmoon           & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.juphoon.justalk}{JusTalk}}            & none                                                                                 & \newmoon                                                           & \fullmoon           & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.safeum.android}{SafeUM}}              & e2ee                                                                                 & \fullmoon                                                          & \fullmoon           & \newmoon          & \fullmoon     & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.yallatech.yallachat}{YallaChat}}      & e2ee                                                                                 & \fullmoon                                                          & \fullmoon           & \newmoon          & \newmoon      & \fullmoon         \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.is.core.app}{Comera}}                 & Push-to-Sync                                                                         & \fullmoon                                                          & \fullmoon           & \fullmoon         & \fullmoon     & \newmoon          \\ \hline
\multicolumn{2}{l}{\href{https://play.google.com/store/apps/details?id=com.wire}{Wire}}                          & Push-to-Sync                                                                         & \fullmoon                                                          & \newmoon            & \newmoon          & \fullmoon     & \fullmoon         \\ \hline
\end{tabular}
\caption{This table contains all analyzed apps, for which we observed personal information leakage to FCM servers in the process of delivering push notifications. The specific observed category of data is indicated by \newmoon~(evidence) and \fullmoon~(no evidence).}
\label{table:broken_promises}
\end{table*}

==> paper/8_conclusion.tex <==
%-------------------------------------------------------------------------------
\section{Conclusion}
\label{sec:conclusion}
%-------------------------------------------------------------------------------



==> scratchbook.tex <==
% INTRODUCTION %

% Why is third-party SDKs/services fundamental?
% The complexity of modern software engineering projects necessitates the reuse of knowledge and code from previously implemented systems. This practice avoids the costs associated with the implementation of complex or boilerplate code, while improving the maintainability of overall systems. In the context of mobile app development, developers rely on third-party tools known as software development kits (SDKs), which include libraries, documentation, code samples, processes, and guides that developers can use and integrate into their own apps~\cite{salza2020third}. For example, the Android SDK is a set of development tools used specifically for developing apps for the Android platform.

% Introduce push notification services. TODO: rephrase as wording taken from FOCI paper.
% A clear example of a functionality that greatly benefits from the reuse of knowledge and code during software development is push notification. Push notifications (also known as cloud messaging) enable applications to transmit time-sensitive information directly to end users of both desktop, browser, and mobile apps. These services have seen widespread adoptions in recent years, with over 600 billion messages sent to 2 billion users in H1 2021 from one provider alone~\cite{?}. Examples of providers include Google's Firebase Cloud Messaging (FCM) and Apple's Push Notification Service (APNS).


% What risks does such a setup present?
% While the benefits of push notification SDKs are undeniable, they also present tangible privacy and security risks to users and legal compliance risks to app vendors. Prior work has investigated the risk of transmitting malware to users via push messaging~\cite{?} and the visibility of personal information in arriving notifications on user's device screen~\cite{?}. Less clear, however, are the privacy compliance risks that app vendors are exposed to by transmitting personal information of users via third-party servers. 

% The recently-introduced comprehensive privacy laws, such as the General Data Protection Regulation (GDPR) in Europe or the California Consumer Privacy Act (CCPA) in California, impose additional obligations on companies who collect, process, and share personal information of individuals. App and website vendors, in particular, are responsible for ensuring that the processing of users' personal information via third-party services and SDKs is lawful, while also informing their users and providing them with the ability to exercise their rights over their personal information.

% What is our research hypothesis?


% What are our research questions?
% In this work, we highlight this issue by focusing on the push messaging functionality provided by Google's Firebase Cloud Messaging (FCM or Firebase) SDK and other third-party cloud messaging providers commonly used by Android app developers. Given the lack of prior work addressing the privacy compliance risks of using third-party push notifications services by Android app developers, we posed the following research questions:
% \begin{itemize}
%   \item \textbf{RQ1:} What are the practices associated with using push notification services provided by platform owners and other third parties?
%   \item \textbf{RQ2:} What mitigation strategies, if any, do app developers employ to protect users' personal information sent as part of push notification messages?
%   \item \textbf{RQ3:} How do app vendors disclose the usage of third-party push notification services for sending users' personal information?
% \end{itemize}

% What did we do?
% To answer these questions, we performed static and dynamic analysis of \analyzedSecureAppCount{} instant messaging (IM) and banking apps to observe information being sent over Google's Firebase infrastructure and handled by the client Android app. We also determined whether information being displayed to the user is potentially sensitive and, if so, whether the app developer has implemented technical solutions (i.e., end-to-end encryption) to safeguard the contents or avoided sending sensitive data using push notifications in the first place. Finally, we examined the privacy policies, privacy labels, and other legal and voluntary disclosures made by app developers to understand whether their practices are being accurately and sufficiently disclosed. 

% What did we find?
% We found that, despite the privacy compliance risks for Android app vendors reliant on Google’s cloud infrastructure to deliver the push messages, the majority of examined app developers sending push notifications with sensitive information to end users do not employ any safeguards to protect the information sent via cloud messaging. In particular, \TODO{note particular numbers here in 1-2 sentences}. Furthermore, we found that the majority of developers do not disclose the usage of third-party push notification services or the personal information that is being shared for the purposes of transmitting push messages. More specifically, \TODO{note particular numbers here in 1-2 sentences}. 

% What are the implications and contributions of our paper?
% Our findings hold important implications not just for the design of Firebase SDK but for the wider third-party tooling ecosystem prevalent in modern software development. Although privacy laws based on FIPPs—such as the GDPR and CCPA—emphasize notice and choice, end users and developers (who are responsible for information practices of their apps and any SDKs they embed) lack the awareness, incentives, and bargaining power to influence the design of the upstream SDKs they employ. As such, we advocate for privacy regulations that shift the burden of data protection from individual developers and users to vendors of SDKs and other market players most capable of taking action to mitigate downstream privacy risks. The specific contributions of our work are as follows:
% \begin{itemize}
%   \item \TODO{Contribution 1.}
%   \item \TODO{Contribution 2.}
%   \item \TODO{Contribution 3.}
% \end{itemize}


% We highlight this issue by focusing on the push messaging functionality provided by Firebase SDK. Firebase SDK provides an efficient solution for implementing push notifications but introduces privacy risks for end users and compliance risks for developers by relying on Google’s cloud infrastructure to deliver the push messages. As such, developers are responsible for implementing privacy-enhancing solutions to safeguard the contents of the messages or avoid sending sensitive data using push notifications in the first place. In practice, we find that although Firebase SDK is the most popular push messaging solution for Android, most developers do not use any privacy-enhancing technologies to safeguard the contents of their Firebase push notifications. 

% What risks do third-party services present?
% Unfortunately, the decreased development costs associated with third-party SDKs often come at the expense of privacy and security of users, whose personal information may be inconspicuously accessed and transmitted by the SDKs in violation of privacy regulations, norms, and contractual obligations~\cite{feal2021dont}. Prior research indicates that developers routinely prioritize factors other than privacy when choosing SDKs to embed into their apps. Even when privacy is at the forefront of the development process, the lack of visibility, documentation, and adequate control of privacy-threatening behaviors of SDKs contributes to heightened privacy risks for users and compliance risks for app developers~\cite{alomar2022developers}. \TODO{Mention the recent regulatory actions and fines against businesses using SDKs?}

% As such, vendors of SDKs possess a particular power in defining the information practices of the apps that employ it. For instance, changing the default configuration of an SDK to collect less data from users would benefit all the downstream apps that use the SDK with the default settings. Even though vendors of SDKs can prioritize privacy in the design of their tools, the economics of modern software engineering entail that vendors who provide privacy-friendly SDKs would be outperformed by SDKs which use agile and data-driven development processes. In the long run, vendors of popular SDKs become even more entrenched in the digital marketplace, as they benefit from the economies of scale afforded by the data collected as a result of the SDK usage.

% In this work, we present a comprehensive end-to-end study of Android’s push notification behavior in practice. The specific contributions of this work are the following:

% BACKGROUND %

% The push notification service needs to know the address of the specific user agent to forward messages from the server to the correct client. During the \textit{registration} or \textit{subscription} phase, the client sends a network request with a unique app identifier to a push service, which generates subscription information associated with the specific app instance and returns it to the client. The client app then typically sends the subscription data to the app server, which stores it in a database. Whenever the server wants to send a push message to a client app, it includes the subscription data in a request to the push service, which can then forward the message to the correct client app instance. See Figure~\ref{fig:registration} for an illustration of the process.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{assets/figures/registration.jpg}
%   \caption{A step-wise depiction of the token registration process. \TODO{Change for FCM.}}
%   \label{fig:registration}
% \end{figure}

% This process differs slightly depending on the type of an app. For web apps, a push service typically provides an endpoint in response to a request from a web client, which the server uses to send push messages to. On the other hand, Google's Firebase push service returns a registration token, which the server includes in the request payload alongside the message sent to the FCM push service, which then uses the token to correctly identify the recipient. Unless stated otherwise, we will refer to the process used by Google's FCM service for registering and sending push messages for the remainder of the paper. 

% % What are the advantages of push messaging?
% Push messaging infrastructure generally employs the publisher-subscriber messaging pattern. Such an architecture holds several advantages over direct server-to-client communication~\cite{?}. First, individual apps maintaining separate long-term connections to their servers would incur significant overhead costs, especially on embedded and mobile devices with limited resources. Second, as the number of app users increases, so does the complexity of maintaining point-to-point connection between the app server and each client app instance. Third, the push service handles cases when client apps are offline, by storing messages and retrying delivery for a predefined amount of time. Fourth, the API exposed by a push service is the same for all apps using the service, enabling better knowledge-sharing and documentation. Finally, many proprietary push services can be configured to collect additional analytics, which can inform developers about the performance of their apps. 

% % https://datatracker.ietf.org/doc/rfc8599/
% Major web browsers (e.g., Google Chrome, Mozilla Firefox, Microsoft Edge) implement the W3C Push API standard for web push notifications~\cite{?}, which allows developers to subscribe client apps and send push messages using standardized web push protocol requests, irrespective of the specific push service, browser, or platform being used. The Push API specification assumes the usage of Internet Engineering Task Force's (IETF) RFC 8030~\cite{?} standard for the delivery of real-time events to user agents and the RFC 8291~\cite{?} standard for the end-to-end encryption of the contents of web push messages to protect against untrusted push services. Although the standardized Push API is supported by mobile browsers~\cite{?}, native mobile applications rely on their platform owner's proprietary mechanisms and protocols. Crucially, neither Apple's Push Notification Service nor Google's Firebase Cloud Messaging solution implement the end-to-end encryption of mobile push notifications contents, which has implications for security and privacy of end users. 

% \subsection{Privacy Implications of Push Messaging}
% Although the design of push notifications presents considerable advantages over alternative approaches (see Section~\ref{sec:background}) and can often provide valuable user experience, there are several important privacy considerations that developers have to be aware when sending push notifications using a push service: 

% \textbf{Informed Consent.} App vendors are required to inform their users and seek their consent before using a third-party push service, such as Google's Firebase, to deliver messages from the app server to its client. Informed consent can be achieved by disclosing the usage and purpose of a push service in the app's privacy policy and then seeking user consent before enabling any data collection by the embedded push notification SDK. This is particularly crucial when sending push notifications for non-essential purposes, such as marketing. 

% It is important to note that Android versions prior to Android 13 (API level 33) did not support runtime permissions for sending push notifications. Therefore, developers have to ensure that they implement correct consent mechanisms to appropriately request permission to send notifications to users running Android versions 12 and below. 

% \textbf{Deceptive Practices.} Vendors must not make material representations that contradict the actual information practices of their apps. In the context of push notifications, this may include developers stating that no personal information is shared with third parties, while transmitting such data in push notifications using third-party push services. 

% \textbf{Data Minimization.} Many data protection regulations around the world, including the EU's General Data Protection Regulation (GDPR) and the California Consumer Privacy Act (CCPA, as amended) require entities processing personal information to adhere to the principles of data minimization, proportionality, and necessity. In other words, the processing and sharing of personal information should be kept to an absolute minimum required for the purpose of delivering push notifications.

% Several push service providers, including Apple and Microsoft (but, notably, not Google) advise developers against sending any sensitive information in the payload of push notifications~\cite{?}. Instead, Microsoft suggests adopting a \textit{push-to-sync} strategy wherein the push message contains only a unique message identifier without any personal information. On receiving the push message, the client app can then request the required information directly from the app server. If the developer requires sending sensitive information in the payload of the push message (e.g., to avoid latency) then Apple recommends end-to-end encryption of contents. 

% \textbf{International Data Transfers.} Another issue relevant to certain data protection laws is the transfer of personal information of individuals to countries outside of their jurisdiction. For instance, the GDPR mandates adequate level of protection for the transfers of personal information of European natural persons outside of EU, for instance, to the United States. Some push services, including Firebase Cloud Messaging, may transfer Europeans' personal information outside of the EU, where it may be subject to a variety of laws that allow government agencies to request the disclosure of user information for civil, administrative, criminal, and national security purposes without the necessary legal protections afforded by the GDPR.

% % \subsection{Push Notification Service Providers}
% % Apple and Google are the leaders in the push messaging feature. In 2009, Apple launched the first-ever push notification service – Apple Push Notification Service (APNs). The next year, Google launched its Cloud to Device Messaging service (C2DM). In October 2014, Google acquired Firebase; it merged with Google’s push messaging service and became known as Firebase Cloud Messaging (FCM).

% % \textbf{Firebase Cloud Messaging (FCM).} ...

% % \TODO{Create a table that compares the most popular push notification providers (+custom provider with MQTT?) and includes information about which ones rely on FCM under the hood.}




% DISCUSSION %
%The overwhelming usage of FCM among Android applications has several important implications. This dependency suggests that a majority of Android applications are tied to Google's infrastructure and ecosystem. This potentially leads to concerns about vendor lock-in, where changes in FCM's policies, pricing, or functionality could have broad implications for a large number of applications.

% \subsection{FCM Market Dominance}
% Our analysis has demonstrated the significant reliance of Android app developers on Google's Firebase Cloud Messaging (FCM) push service. This reliance manifests itself in the vast majority of Android apps using Google's infrastructure to send push notifications to their users. While alternatives to FCM exist, including ones that do not rely on Google's push service, we found that the uptake of these options is relatively low. A number of factors contribute to this state of affairs, with one of the most prominent being the inherent appeal of Google's all-encompassing ecosystem. By offering a wide variety of integrated services, Google has created an ecosystem that is difficult for developers to resist. The convenience of FCM, its native integration with Android, its robust performance, and its associated analytics and diagnostic tools, make it an attractive choice for developers, especially when compared to alternatives that may not offer such an extensive range of functionalities.

% At the same time, developers reliant on Google's FCM push service expose themselves to heightened risks of noncompliance with privacy regulations, while also contributing to elevated risks of privacy harms for their end users. First, the lack of in-built support for end-to-end encryption of push message contents, which stands in contrast to the default encryption of payloads of web push notifications. Although developers can transmit the only message identifier via Firebase and fetch the remaining content directly from the app server, we found that in practice few choose do so. Instead, many developers directly transmit the information required to display the push notification using Google's infrastructure, even if that information is sensitive or protected under privacy law. Second, we found prevalence of default settings set by Google's Firebase API, including lengthy message retention periods and auto-initialization of the SDK, which contribute to violations of the principle of Privacy by Default (PbD) among Android app developers. 

% The high degree of market dominance enjoyed by FCM, as demonstrated by our findings, highlights a broader issue in the Android ecosystem - the significant influence of Google. The combination of Google's massive resource base and its dominance over the Android operating system has made it possible for Google to set the bar high for any potential new entrants. This monopolistic scenario could stifle competition and innovation in the market for push notification services. A more competitive market would likely result in better privacy protections and service offerings for users, driven by the need for differentiating features and value propositions among competitors.

% \subsection{Privacy and Third-Party SDKs}
% Our research highlights a broader issue that exists in the mobile app ecosystem, namely, the privacy implications associated with third-party SDKs and tools used by app developers. Privacy regulations state that app developers, who dictate the means and the purposes of data processing, are generally responsible for the information practices of the SDKs they integrate into their apps~\cite{?}. This includes how the SDKs collect, process, and distribute user personal information. However, prior research has demonstrated that developers often lack a comprehensive understanding of the intricate details of these practices~\cite{?}. Their focus is typically geared towards leveraging SDKs to enhance app functionality or user experience, rather than scrutinizing the privacy ramifications of the SDKs they use. This issue is often compounded by the default settings of many SDKs, which often are not privacy-centric~\cite{?}. Research in other fields, including behavioral economics, has already widely acknowledged that default settings are ``sticky''---that is, individuals are less likely to alter them even if there are better choices available~\cite{?}. Consequently, if an SDK’s default setting permits extensive data collection or sharing, developers may inadvertently permit these practices, leading to potential privacy violations.

% Beyond these identified concerns, there may well be other problems associated with third-party SDKs. For example, the sheer volume of SDKs available can make it challenging for developers to assess the privacy compliance of each one thoroughly. Also, some SDKs might collect excessive user data under the guise of providing better functionality, thus violating the data minimization principle of privacy regulations. We, therefore, welcome the upcoming efforts by both Google~\cite{?} and Apple~\cite{?} to compile lists of third-party SDKs alongside their information practices. Nevertheless, these practices are declared by SDK vendors themselves and it is unclear to what extent Google and Apple would audit the conformity of SDKs with their stated practices. 

% Addressing these issues requires a multifaceted approach. While individual developers indeed have a role to play in ensuring privacy compliance, the responsibility should not lie solely with them. Vendors of SDKs need to shoulder some of the burden by setting privacy-conscious defaults and providing clear, comprehensive information about their data practices. Moreover, platform owners like Google and Apple have a significant role to play. They can help improve the privacy landscape by auditing the SDKs used in apps on their platforms and providing clear guidelines and tools for developers to ensure privacy compliance. Such an approach would serve to educate developers about privacy risks and provide them with practical measures to mitigate these risks. Additionally, regulations should focus not only on the liability of individual developers but also on the vendors of SDKs and platform owners. This could manifest as regulatory measures that mandate privacy audits of SDKs, penalties for non-compliance, or requirements for transparent disclosure of data practices.

% \subsection{Recommendations}
% We conclude our discussion with a set of recommendations for improving the existing mobile app ecosystem. We emphasize that the issue of preserving privacy in mobile apps requires efforts from different stakeholders, including end users, app developers, SDK vendors, platform owners, and regulators.  

% We believe that developers should strive to better understand the privacy implications of the third-party SDKs they utilize, especially regarding data collection, processing, and sharing. Additionally, developers should take responsibility for adjusting SDK default settings that may not prioritize privacy and ensuring their apps are compliant with applicable privacy regulations. Furthermore, vendors of SDKs are recommended to prioritize privacy in their SDK offerings. This could include setting privacy-conscious defaults, providing clear and transparent information about their data practices, and actively helping developers understand and navigate the privacy implications of using their SDKs.

% As gatekeepers, platform owners such as Google and Apple are recommended to enforce stricter privacy guidelines on their app stores. They could implement routine audits of apps and SDKs for privacy compliance, provide tools and resources to assist developers in creating privacy-compliant apps, and promptly remove apps found to be in violation of privacy standards. Moreover, regulators should consider revising current regulations to extend liability beyond individual developers to SDK vendors and platform owners. Regulatory measures could include mandatory privacy audits of SDKs, hefty penalties for non-compliance, or requirements for transparent disclosure of data practices. Finally, regulators might also consider promoting existing privacy-focused standards (e.g., RFC 8291 for encrypted contents of push notifications), as well as the development of new standards and best practices for the mobile app industry.
